Density of asteroids

A considerable amount of information regarding the processes that occurred during the accretion of the early planetesimals is still present among the small bodies of our solar system. A review of our current knowledge of the density of small bodies is presented here. Intrinsic physical properties of small bodies are sought by searching for relationships between the dynamical and taxonomic classes, size, and density. Mass and volume estimates for 287 small bodies are collected from the literature. The accuracy and biases affecting the methods used to estimate these quantities are discussed and best-estimates are strictly selected. Bulk densities are subsequently computed and compared with meteorite density, allowing to estimate the macroporosity within these bodies. Dwarf-planets apparently have no macroporosity, while smaller bodies can have large voids. This trend is apparently correlated with size: C and S-complex asteroids tends to have larger density with increasing diameter. The average density of each Bus-DeMeo taxonomic classes is computed. S-complex asteroids are more dense on average than those in the C-complex that in turn have a larger macroporosity, although both complexes partly overlap. Within the C-complex, B-types stand out in albedo, reflectance spectra, and density, indicating a unique composition. Asteroids in the X-complex span a wide range of densities, suggesting that many compositions are included in the complex. Comets and TNOs have high macroporosity and low density, supporting the current models of internal structures made of icy aggregates. The number of density estimates sky-rocketed during last decade from a handful to 287, but only a third of the estimates are more precise than 20%. Several lines of investigation to refine this are contemplated, including observations of multiple systems, 3-D shape modeling, and orbital analysis from Gaia astrometry.

==> app-figs/figDiam-000033.tex <==
\begin{figure}[!ht]
  \centering
  \includegraphics[width=.49\textwidth]{diam000033.pdf}
\caption[Diameter estimates for (33) Polyhymnia]{%
  \label{fap: diam000033}
  Diameter estimates for (33) Polyhymnia.
}
\end{figure}


==> app-figs/figDiam-000675.tex <==
\begin{figure}[!ht]
  \centering
  \includegraphics[width=.49\textwidth]{diam000675.pdf}
\caption[Diameter estimates for (675) Ludmilla]{%
  \label{fap: diam000675}
  Diameter estimates for (675) Ludmilla.
  See~\ref{app: biblio} for the references, and Fig.~\ref{fap: diam81P/Wild2} for symbols key.
}
\end{figure}


==> app-figs/figDiam-un000001.tex <==
\begin{figure}[!ht]
  \centering
  \includegraphics[width=.49\textwidth]{diam-un000001.pdf}
\caption[Diameter estimates for 81P/Wild2]{%
  \label{fap: diam81P/Wild2}
  Diameter estimates for 81P/Wild2.
  See~\ref{app: biblio} for the references, and Fig.~XXX for symbols key.
}
\end{figure}


==> app-figs/figDiam-un000007.tex <==
\begin{figure}[!ht]
  \centering
  \includegraphics[width=.49\textwidth]{diam-un000007.pdf}
\caption[Diameter estimates for 67P/C-G]{%
  \label{fap: diam67P/C-G}
  Diameter estimates for 67P/C-G.
  See~\ref{app: biblio} for the references, and Fig.~XXX for symbols key.
}
\end{figure}


==> app-figs/figDiam-un000008.tex <==
\begin{figure}[!ht]
  \centering
  \includegraphics[width=.49\textwidth]{diam-un000008.pdf}
\caption[Diameter estimates for 81P/Wild2]{%
  \label{fap: diam81P/Wild2}
  Diameter estimates for 81P/Wild2.
  See~\ref{app: biblio} for the references, and Fig.~XXX for symbols key.
}
\end{figure}


==> app-figs/figDiam-un000010.tex <==
\begin{figure}[!ht]
  \centering
  \includegraphics[width=.49\textwidth]{diam-un000010.pdf}
\caption[Diameter estimates for 2P/Encke]{%
  \label{fap: diam2P/Encke}
  Diameter estimates for 2P/Encke.
}
\end{figure}


==> app-figs/figDiam-un000011.tex <==
\begin{figure}[!ht]
  \centering
  \includegraphics[width=.49\textwidth]{diam-un000011.pdf}
\caption[Diameter estimates for 2P/Encke]{%
  \label{fap: diam2P/Encke}
  Diameter estimates for 2P/Encke.
}
\end{figure}


==> app-figs/figDiam-un000012.tex <==
\begin{figure}[!ht]
  \centering
  \includegraphics[width=.49\textwidth]{diam-un000012.pdf}
\caption[Diameter estimates for 9P/Tempel1]{%
  \label{fap: diam9P/Tempel1}
  Diameter estimates for 9P/Tempel1.
}
\end{figure}


==> app-figs/figDiam-un000013.tex <==
\begin{figure}[!ht]
  \centering
  \includegraphics[width=.49\textwidth]{diam-un000013.pdf}
\caption[Diameter estimates for 9P/Tempel1]{%
  \label{fap: diam9P/Tempel1}
  Diameter estimates for 9P/Tempel1.
}
\end{figure}


==> app-figs/figDiam-un000017.tex <==
\begin{figure}[!ht]
  \centering
  \includegraphics[width=.49\textwidth]{diam-un000017.pdf}
\caption[Diameter estimates for 2P/Encke]{%
  \label{fap: diam2P/Encke}
  Diameter estimates for 2P/Encke.
}
\end{figure}


==> app-figs/figDiam-un000019.tex <==
\begin{figure}[!ht]
  \centering
  \includegraphics[width=.49\textwidth]{diam-un000019.pdf}
\caption[Diameter estimates for 9P/Tempel1]{%
  \label{fap: diam9P/Tempel1}
  Diameter estimates for 9P/Tempel1.
}
\end{figure}


==> app-figs/figDiam-un000025.tex <==
\begin{figure}[!ht]
  \centering
  \includegraphics[width=.49\textwidth]{diam-un000025.pdf}
\caption[Diameter estimates for 67P/C-G]{%
  \label{fap: diam67P/C-G}
  Diameter estimates for 67P/C-G.
}
\end{figure}


==> app-figs/figMass-un000001.tex <==
\begin{figure}[!ht]
  \centering
  \includegraphics[width=.49\textwidth]{mass-un000001.pdf}
\caption[Mass estimates for 9P/Tempel1]{%
  \label{fap: mass9P/Tempel1}
  Mass estimates for 9P/Tempel1.
  See~\ref{app: biblio} for the references.
}
\end{figure}


==> app-figs/figMass-un000012.tex <==
\begin{figure}[!ht]
  \centering
  \includegraphics[width=.49\textwidth]{mass-un000012.pdf}
\caption[Mass estimates for 9P/Tempel1]{%
  \label{fap: mass9P/Tempel1}
  Mass estimates for 9P/Tempel1.
}
\end{figure}


==> app-figs/figMass-un000013.tex <==
\begin{figure}[!ht]
  \centering
  \includegraphics[width=.49\textwidth]{mass-un000013.pdf}
\caption[Mass estimates for 9P/Tempel1]{%
  \label{fap: mass9P/Tempel1}
  Mass estimates for 9P/Tempel1.
}
\end{figure}


==> app-figs/figMass-un000019.tex <==
\begin{figure}[!ht]
  \centering
  \includegraphics[width=.49\textwidth]{mass-un000019.pdf}
\caption[Mass estimates for 9P/Tempel1]{%
  \label{fap: mass9P/Tempel1}
  Mass estimates for 9P/Tempel1.
}
\end{figure}

